Toward a Programmable FIB Caching Architecture

The current Internet routing ecosystem is neither sustainable nor economical. More than 711K IPv4 routes and more than 41K IPv6 routes exist in current global Forwarding Information Base (FIBs) with growth rates increasing. This rapid growth has serious consequences, such as creating the need for costly FIB memory upgrades and increased potential for Internet service outages. And while FIB memories are power-hungry and prohibitively expensive, more than 70\% of the routes in FIBs carry no traffic for long time periods, a wasteful use of these expensive resources. Taking advantage of the emerging concept of programmable data plane, we design a programmable FIB caching architecture to address the existing concerns. Our preliminary evaluation results show that the architecture can significantly mitigate the global routing scalability and poor FIB utilization issues.

==> Makefile <==
PRJ = aggregate

# to use eps figures
DVIOPT = -P cmz -t letter -G0

all : viewpdf 

#${PRJ}.dvi : *.tex *.bib 
#	pdflatex ${PRJ}; bibtex ${PRJ}; pdflatex ${PRJ}; pdflatex ${PRJ} 
#
#${PRJ}.ps : ${PRJ}.dvi
#	dvips ${DVIOPT} -o ${PRJ}.ps ${PRJ}.dvi

#${PRJ}.pdf : ${PRJ}.ps
${PRJ}.pdf : *.tex *.bib 
	pdflatex ${PRJ}; bibtex ${PRJ}; pdflatex ${PRJ}; pdflatex ${PRJ} 
#	ps2pdf ${PRJ}.ps ${PRJ}.pdf

dvi : ${PRJ}.dvi

ps : ${PRJ}.ps

pdf : ${PRJ}.pdf

viewdvi : ${PRJ}.dvi
	xdvi ${PRJ}.dvi &

viewps : ${PRJ}.ps
	open ${PRJ}.ps &

viewpdf : ${PRJ}.pdf
	open ${PRJ}.pdf &

# to use non-eps figures.
#all : view 

#${PRJ}.pdf : *.tex 
#	pdflatex ${PRJ}; bibtex ${PRJ}; pdflatex ${PRJ}; pdflatex ${PRJ}

#pdf: ${PRJ}.pdf

#view : ${PRJ}.pdf
#	open ${PRJ}.pdf &

pack : pdf
	/bin/rm -f ../${PRJ}.tgz; tar -zcf ../${PRJ}.tgz Makefile *.tex IEEEtran.cls net.bib ${PRJ}.pdf figure 

clean:
	/bin/rm -f *.toc *.aux *.bbl *.blg *.log *.dvi *~* *.bak ${PRJ}.pdf ${PRJ}.ps

distclean:
	/bin/rm -f *.toc *.aux *.bbl *.blg *.log ${PRJ}.dvi ${PRJ}.ps ${PRJ}.pdf *~* *.bak

#cut : ${PRJ}.dvi 
#	dvips -t letter -o summary.ps -p=2 -l=2 ${PRJ}.dvi
#	ps2pdf summary.ps summary.pdf
#	/bin/rm summary.ps \
#
#	dvips -t letter -o description.ps -p=3 -l=17 ${PRJ}.dvi
#	ps2pdf description.ps description.pdf
#	/bin/rm description.ps \
#
#	dvips -t letter -o references.ps -p=18 -l=20 ${PRJ}.dvi
#	ps2pdf references.ps references.pdf
#	/bin/rm references.ps


